Probing Parity-Violation with the Four-Point Correlation Function of BOSS Galaxies

Parity-violating physics in the early Universe can leave detectable traces in late-time observables. Whilst vector- and tensor-type parity-violation can be observed in the $B$-modes of the cosmic microwave background, scalar-type signatures are visible only in the four-point correlation function (4PCF) and beyond. This work presents a blind test for parity-violation in the 4PCF of the BOSS CMASS sample, considering galaxy separations in the range $[20,160]h^{-1}\mathrm{Mpc}$. The parity-odd 4PCF contains no contributions from standard $\Lambda$CDM physics and can be efficiently measured using recently developed estimators. Data are analyzed using both a non-parametric rank test (comparing the BOSS 4PCFs to those of realistic simulations) and a compressed $\chi^2$ analysis, with the former avoiding the assumption of a Gaussian likelihood. These find similar results, with the rank test giving a detection probability of $99.6\%$ ($2.9\sigma$). This provides significant evidence for parity-violation, either from cosmological sources or systematics. We perform a number of systematic tests: although these do not reveal any observational artefacts, we cannot exclude the possibility that our detection is caused by the simulations not faithfully representing the statistical properties of the BOSS data. Our measurements can be used to constrain physical models of parity-violation. As an example, we consider a coupling between the inflaton and a $U(1)$ gauge field and place bounds on the latter's energy density, which are several orders of magnitude stronger than those previously reported. Upcoming probes such as DESI and Euclid will reveal whether our detection of parity-violation is due to new physics, and strengthen the bounds on a variety of models.

==> old.tex <==
\section{Derivation of the Chern-Simons 4PCF Model}\label{appen: chern-simons}

\oliver{is this theory IR safe? seems to be divergent as $|\vk_1+\vk_2|\to0$.}

Here, we sketch the derivation of the parity-odd trispectrum discussed in \S\ref{sec: inflationary-model}. Our starting point is the general expression given in \eqref{eq: CS-4PCF-overall}, which is a product of four pieces. By expressing each contribution in terms of isotropic basis functions, we may compute the full 4PCF model in an efficient manner.

First, consider the Dirac delta function. This may be written in terms of the isotropic basis functions of \textit{four} coordinates, $\P_{\ell_1\ell_2(\ell_{12})\ell_3\ell_4}(\hk_1,\hk_2,\hk_3,\hk_4)$, as 
\beq\label{eq: Dirac-expansion}
    (2\pi)^3\delta_{\rm D}(\vk_1+\vk_2+\vk_3+\vk_4) &=& (4\pi)^3\sum_{\ell_1\ell_2\ell_{12}\ell_3\ell_4}i^{\ell_1+\ell_2+\ell_3+\ell_4}\int s^2ds\,\prod_{i=1}^4\left[j_{\ell_i}(k_is)\right]\tjo{\ell_1}{\ell_2}{\ell_{12}}\tjo{\ell_{12}}{\ell_3}{\ell_4}
    \\\nonumber
    &&\,\times\,(-1)^{\ell_{12}}\left[\frac{(2\ell_1+1)(2\ell_2+1)(2\ell_3+1)(2\ell_4+1)}{2\ell_{12}+1}\right]^{1/2}\P_{\ell_1\ell_2(\ell_{12})\ell_3\ell_4}(\hk_1,\hk_2,\hk_2,\hk_3,\hk_4),
\eeq
where $j_\ell(x)$ is a spherical Bessel function. This can be shown by writing the Dirac function as the $\vs$ integral of $\mathrm{exp}\left[-i\vs\cdot(\vk_1+\vk_2+\vk_3+\vk_4)\right]$, expanding the complex exponentials via the plane wave identity, integrating over the angular parts of $\vs$ by introducing two Gaunt integrals, and simplifying, using 3-$j$ identities. Note that \eqref{eq: Dirac-expansion} is separable in $k_i$, following the one-dimensional $s$ integral.

Secondly, we may write the transfer piece (involving $M(k)Z_1(\vk)$) by first noting that $Z_1(\vk)$ can be expanded in spherical harmonics as
\beq
    Z_1(\vk) = 4\pi\sum_{\ell m}\left[\left(b+\frac{f}{3}\right)\delta^{\rm K}_{\ell 0}+\frac{2f}{15}\delta^{\rm K}_{\ell 2}\right]Y^{}_{\ell m}(\hk)Y^*_{\ell m}(\hn) \equiv 4\pi\sum_{\ell m}Z^{}_\ell Y^{}_{\ell m}(\hk)Y^*_{\ell m}(\hn),
\eeq
where $\hn$ is some line of sight (LoS), $b$ is the linear bias and $f$ is the growth rate, and we have used the Legendre polynomial addition theorem to convert a Legendre polynomial into spherical harmonics. The product of four functions can thus be written
\beq
    \prod_{i=1}^4\left[M(k_i)Z_1(\vk_i)\right] &=& (4\pi)^4\sum_{\ell_1\ell_2\ell_3\ell_4}\sum_{\ell_{12}}\prod_{i=1}^4\left[M(k_i)Z_{\ell_i}\right]\P_{\ell_1\ell_2(\ell_{12})\ell_3\ell_4}(\hk_1,\hk_2,\hk_3,\hk_4)\P^*_{\ell_1\ell_2(\ell_{12})\ell_3\ell_4}(\hn,\hn,\hn,\hn),
\eeq
involving isotropic functions of both $\hk_i$ and the LoS $\hn$. Since we consider only isotropic 4PCFs, we can integrate over the LoS (which is equivalent to performing a joint rotation of all $\hk_i$). Following some algebra, this gives
\beq\label{eq: transfer-expansion}
    \int \frac{d\hn}{4\pi} \prod_{i=1}^4\left[M(k_i)Z_1(\vk_i)\right] &=& (4\pi)^2\sum_{\ell_1\ell_2\ell_3\ell_4}\sum_{\ell_{12}}\prod_{i=1}^4\left[M(k_i)Z_{\ell_i}\right](-1)^{\ell_1+\ell_2+\ell_3+\ell_4}(-1)^{\ell_{12}}\P_{\ell_1\ell_2(\ell_{12})\ell_3\ell_4}(\hk_1,\hk_2,\hk_2,\hk_3,\hk_4)\nonumber\\
    &&\,\times\,\left[\frac{(2\ell_1+1)(2\ell_2+1)(2\ell_3+1)(2\ell_4+1)}{2\ell_{12}+1}\right]^{1/2}\tjo{\ell_1}{\ell_2}{\ell_{12}}\tjo{\ell_{12}}{\ell_3}{\ell_4},
\eeq
which is again separable in $k_i$.

Thirdly, consider the form of the trispectrum itself, as defined in \eqref{eq: tk-CS}. For this, it is easiest to work in basis functions of three-positions, \textit{i.e.} $\P_{\ell_1\ell_2\ell_3}(\hk_1,\hk_2,\hk_3)$, then convert using $\P_{\ell_1\ell_2\ell_3}(\hk_1,\hk_2,\hk_3) = \sqrt{4\pi}\P_{\ell_1\ell_2(\ell_3)\ell_30}(\hk_1,\hk_2,\hk_3,\hk_4)$. The trispectrum contains a number of pieces of interest. Firstly, the triple-product is proportional to:
\beq\label{eq: triple-product}
    (\hk_1\times\hk_3)\cdot\hk_2 = -i\frac{\sqrt{2}}{3}(4\pi)^{3/2}\P_{111}(\hk_1,\hk_2,\hk_3)
\eeq
\citep[cf.\,][Appendix A]{2020arXiv201014418C}. The pieces depending on $(\vk_1+\vk_2)$ an be split into two types:
\beq
    \frac{P_\zeta(|\vk_1+\vk_2|)}{|\vk_1+\vk_2|}\left[1-\hk_1\cdot\hk_3+\hk_1\cdot\widehat{\vk_1+\vk_2}-\hk_3\cdot\widehat{\vk_1+\vk_2}\right] &=& \frac{P_\zeta(|\vk_1+\vk_2|)}{|\vk_1+\vk_2|}[1-\hk_1\cdot\hk_3]\\\nonumber
    &&\,+\,\frac{P_\zeta(|\vk_1+\vk_2|)}{|\vk_1+\vk_2|^2}\left[k_1+\hk_1\cdot\hk_2-k_1\hk_3\cdot\hk_1-k_2\hk_3\cdot\hk_2\right].
\eeq
Combining with \eqref{eq: triple-product} via the product-to-sum relations \citep[\S6]{2020arXiv201014418C}, allows the angular parts to be written
\beq
    \left[(\hk_1\times\hk_3)\cdot\hk_2\right](1-\hk_1\cdot\hk_3) = -i\frac{\sqrt{2}}{3}(4\pi)^{3/2}\left[\P_{111}(\hk_1,\hk_2,\hk_3)+\P_{212}(\hk_1,\hk_2,\hk_3)\right]
\eeq
and
\beq
    &&\left[(\hk_1\times\hk_3)\cdot\hk_2\right]\left(k_1+(\hk_1\cdot\hk_2)k_2-(\hk_3\cdot\hk_1)k_1-(\hk_3\cdot\hk_2)k_2\right) = -i\frac{\sqrt{2}}{3}(4\pi)^{3/2}\\\nonumber
    &&\quad\times\quad\left[k_1\P_{111}(\hk_1,\hk_2,\hk_3)-\frac{k_2}{\sqrt{5}}\P_{221}(\hk_1,\hk_2,\hk_3)+\frac{k_1}{\sqrt{5}}\P_{212}(\hk_1,\hk_2,\hk_3)+\frac{k_2}{\sqrt{5}}\P_{122}(\hk_1,\hk_2,\hk_3)\right].
\eeq
To compute the pieces depending on $|\vk_1+\vk_2|$, we may use the relation
\beq\label{eq: Pzeta-k12}
    |\vk_1+\vk_2|^{-n}P_\zeta(|\vk_1+\vk_2|) = (4\pi)^{5/2}\sum_L \sqrt{2L+1}\P_{LL0}(\hk_1,\hk_2,\hk_3)\int x^2dx\,\zeta_{-n}(x)j_L(k_1x)j_L(k_2x),
\eeq
where $\zeta_{-n}(x)$ is the Fourier Transform of $k^{-n}P_\zeta(k)$. \oliver{this isn't convergent, unless $n\leq-1$...}To proceed, we combine the basis functions of the angular components with those of \eqref{eq: Pzeta-k12} via
\beq
    \P_{\ell_1\ell_2\ell_3}(\hk_1,\hk_2,\hk_3)\P_{LL0}(\hk_1,\hk_2,\hk_3) &=& \frac{1}{4\pi}\sum_{\ell_1'\ell_2'\ell_3'}(-1)^{\ell_1'+\ell_1+L+\ell_3}\sqrt{(2\ell_1'+1)(2\ell_2'+1)(2\ell_1+1)(2\ell_2+1)(2L+1)}\\\nonumber
    &&\,\times\,\tjo{\ell_1}{L}{\ell_1'}\tjo{\ell_2}{L}{\ell_2'}\begin{Bmatrix}\ell_1 & \ell_1' & L\\ \ell_2' & \ell_2 & \ell_3\end{Bmatrix} \delta^{\rm K}_{\ell_3^{}\ell_3'}\P_{\ell_1'\ell_2'(\ell_3')\ell_3'0}(\hk_1,\hk_2,\hk_3,\hk_4)\\\nonumber
    &\equiv& \sum_{\ell_1'\ell_2'\ell_3'}U_{\ell_1\ell_2\ell_3L}^{\ell_1'\ell_2'\ell_3'}\P_{\ell_1'\ell_2'(\ell_3')\ell_3'0}(\hk_1,\hk_2,\hk_3,\hk_4),
\eeq
using the product-to-sum relations of \citep[\S6]{2020arXiv201014418C}, and simplifying the resulting Wigner 9-$j$ symbol into a 6-$j$ symbol, shown in curly brackets. In full, this allows $t_{\vk_3\vk_4}^{\vk_1\vk_2}$ to be written in a form separable in $k_i$:
\beq\label{eq: tk-expansion}
    t_{\vk_3\vk_4}^{\vk_1\vk_2} &=& -\sqrt{2}(4\pi)^3A_{\rm CS}P_\zeta(k_1)P_\zeta(k_3)\sum_L\sqrt{2L+1}\int 4\pi x^2dx\,j_L(k_1x)j_L(k_2x)\sum_{\ell_1'\ell_2'\ell_3'}\\\nonumber
    &&\,\times\,\left\{\zeta_{-1}(x)\left[U_{111L}^{\ell_1'\ell_2'\ell_3'}+\frac{1}{\sqrt{5}}U_{212L}^{\ell_1'\ell_2'\ell_3'}\right]+\zeta_{-2}(x)\left[k_1U_{111L}^{\ell_1'\ell_2'\ell_3'}-\frac{k_2}{\sqrt{5}}U_{221L}^{\ell_1'\ell_2'\ell_3'}+\frac{k_1}{\sqrt{5}}U_{212}^{\ell_1'\ell_2'\ell_3'}+\frac{k_2}{\sqrt{5}}U_{122L}^{\ell_1'\ell_2'\ell_3'}\right]\right\}\\\nonumber
    &&\,\times\,\P_{\ell_1'\ell_2'(\ell_3')\ell_3'0}(\hk_1,\hk_2,\hk_3,\hk_4).
\eeq

The contributions in \eqref{eq: Dirac-expansion}, \eqref{eq: transfer-expansion}, \& \eqref{eq: tk-expansion} involve three basis functions of the form $\P_{\ell_1\ell_2(\ell_{12})\ell_3\ell_4}(\hk_1,\hk_2,\hk_3,\hk_4)$. These can be combined via generalized Gaunt integrals \citep{2020arXiv201014418C}. Schematically:
\beq
    \P_{\L_1}\P_{\L_2}\P_{\L_3} = \sum_{\L}\mathcal{E}(\L)\left[\sum_{\L'}\mathcal{E}(\L')\mathcal{G}^{\L_1\L_2\L'}\mathcal{G}^{\L'\L_3\L}\right]\P_\L
\eeq
where $\L = \{\ell_1,\ell_2,(\ell_{12}),\ell_3,\ell_4\}$ and $\mathcal{E}(\L) = (-1)^{\ell_1+\ell_2+\ell_3+\ell_4}$. The combined result thus contains only a single basis function.

The final contribution to \eqref{eq: CS-4PCF-overall} is the projection integrals into real space. In particular, we consider the term
\beq\label{eq: projection-term}
   \int\prod_{i=1}^4\frac{d\hk_i}{4\pi}\int d\hr_1d\hr_2d\hr_3\,\P_{\ell_1\ell_2\ell_3}^*(\hr_1,\hr_2,\hr_3)\sum_G\left[e^{i(\vk_{G1}\cdot\vr_1+\vk_{G2}\cdot\vr_2+\vk_{G3}\cdot\vr_3)}\right]\P_{L_1L_2(L_{12})L_3L_4}(\hk_1,\hk_2,\hk_3,\hk_4),
\eeq
inserting an isotropic basis function in $\{\hk_1,\hk_2,\hk_3,\hk_4\}$ (appearing from the above manipulations), and writing the sum over 24 permutations as $\sum_G$, where $\{G1,G2,G3,G4\}$ is some permutation of $\{1,2,3,4\}$. The radial contributions can be written
\beq\label{eq: projection-radial}
    \int d\hr_1d\hr_2d\hr_3\,\P_{\ell_1\ell_2\ell_3}^*(\hr_1,\hr_2,\hr_3)e^{i(\vk_{G1}\cdot\vr_1+\vk_{G2}\cdot\vr_2+\vk_{G3}\cdot\vr_3)} &=& (4\pi)^{7/2}i^{\ell_1+\ell_2+\ell_3}j_{\ell_1}(k_{G1}r_1)j_{\ell_2}(k_{G2}r_2)j_{\ell_3}(k_{G3}r_3)\\\nonumber
    &&\,\times\,\P^*_{\ell_1\ell_2(\ell_3)\ell_30}(\hk_{G1},\hk_{G2},\hk_{G3},\hk_{G4}).
\eeq
Next, we can permute the arguments of the isotropic function as 
\beq\label{eq: permutation}
    \P^*_{\ell_1\ell_2(\ell_3)\ell_30}(\hk_{G1},\hk_{G2},\hk_{G3},\hk_{G4}) &=& \sum_{\L'}\mathcal{B}^G_{\L\L'}\P_{\L'}(\hk_1,\hk_2,\hk_3,\hk_4)\\\nonumber
    &=& (-1)^{\Phi_G} \P^*_{\ell_{H1}\ell_{H2}(L_{12})\ell_{H3}\ell_{H4}}(\hk_1,\hk_2,\hk_3,\hk_4)
\eeq
\citep[\S7]{2020arXiv201014418C}, where we have performed numerous simplifications to obtain the second line, writing $H$ as the inverse permutation of $G$. Here, we note that one of $\{\ell_{H1},\ell_{H2},\ell_{H3}, \ell_{H4}\}$ is zero, and further, that $L_{12} = \ell_{H1}$ if $\ell_{H2}$ is zero, $L_{12} = \ell_{H3}$ if $\ell_{H4}$ is zero, \textit{et cetera}. The phase factor, $\Phi_G$, is $1$ if $\{\ell_{H1},\ell_{H2},\ell_{H3},\ell_{H4}\}$ is an even permutation of $\{1,2,3\}$ (dropping the zero), and $\ell_1+\ell_2+\ell_3$ else. Inserting \eqref{eq: permutation}\,\&\,\ref{eq: projection-radial} into \eqref{eq: projection-term}, we find
\beq
    &&\int\prod_{i=1}^4\frac{d\hk_i}{4\pi}\int d\hr_1d\hr_2d\hr_3\,\P_{\ell_1\ell_2\ell_3}^*(\hr_1,\hr_2,\hr_3)\sum_G\left[e^{i(\vk_{G1}\cdot\vr_1+\vk_{G2}\cdot\vr_2+\vk_{G3}\cdot\vr_3)}\right]\P_{L_1L_2(L_{12})L_3L_4}(\hk_1,\hk_2,\hk_3,\hk_4)\\\nonumber
    &=& \frac{1}{\sqrt{4\pi}}i^{\ell_1+\ell_2+\ell_3}\sum_Gj_{\ell_1}(k_{G1}r_1)j_{\ell_2}(k_{G2}r_2)j_{\ell_3}(k_{G3}r_3)(-1)^{\Phi_H}\delta^{\rm K}_{\ell_{H1}L_1}\delta^{\rm K}_{\ell_{H2}L_2}\delta^{\rm K}_{\ell_{H3}L_3}\delta^{\rm K}_{\ell_{H4}L_4}
\eeq

We finally combine the above results. Defining
\beq\label{eq: 4pcf-CS-defs}
    f_{\ell_1\ell_2(\ell_{12})\ell_3\ell_4} &=& (4\pi)^2\tjo{\ell_1}{\ell_2}{\ell_{12}}\tjo{\ell_{12}}{\ell_3}{\ell_4}(-1)^{\ell_{12}}(-1)^{\ell_{1234}}\left[\frac{(2\ell_1+1)(2\ell_2+1)(2\ell_3+1)(2\ell_4+1)}{2\ell_{12}+1}\right]^{1/2},\\\nonumber
    A_\lambda^1(k,x) &=& \left[\zeta_{-1}(x)+k\zeta_{-2}(x)\right]P_\zeta(k)j_\lambda(kx), \qquad\qquad A_\lambda^2(k,x) = P_\zeta(k)j_\lambda(kx),\\\nonumber
    B_\lambda^1(k,x) &=& j_\lambda(kx), \qquad\qquad B_\lambda^2(k,x) = \zeta_{-2}(x)kj_L(kx),\\\nonumber
    g_{1,\lambda}^{\ell_1\ell_2\ell_3} &=& U_{111\lambda}^{\ell_1\ell_2\ell_3}+\frac{1}{\sqrt{5}}U_{212L}^{\ell_1\ell_2\ell_3}, \qquad\qquad g_{2,\lambda}^{\ell_1\ell_2\ell_3}= \frac{1}{\sqrt{5}}\left(U_{122\lambda}^{\ell_1\ell_2\ell_3}-U_{221\lambda}^{\ell_1\ell_2\ell_3}\right),
\eeq
as well as the $k$-integrals
\beq\label{eq: Q-integrals}
    \mathcal{Q}^{(1)m}_{\ell l\lambda}(r,s,x) &=& \int \frac{k^2dk}{2\pi^2}(-1)^l j_l(ks)M(k)A_{\lambda}^m(k,x)j_\ell(kr)\\\nonumber
    \mathcal{Q}^{(2)m}_{\ell l\lambda}(r,s,x) &=& \int \frac{k^2dk}{2\pi^2}(-1)^l j_l(ks)M(k)B_{\lambda}^m(k,x)j_\ell(kr)\\\nonumber
    \mathcal{Q}^{(3)}_{\ell l}(r,s) &=& \int \frac{k^2dk}{2\pi^2}(-1)^l j_l(ks)M(k)P_\zeta(k)j_\ell(kr)\\\nonumber
    \mathcal{Q}^{(4)}_{\ell l}(r,s) &=& \int \frac{k^2dk}{2\pi^2}(-1)^l j_l(ks)M(k)j_\ell(kr)\\\nonumber
\eeq
the 4PCF may be written
\beq\label{eq: 4pcf-CS-full-model}
    \zeta_{\ell_1\ell_2\ell_3}(r_1,r_2,r_3) &=& -\sqrt{2}(4\pi)^{3/2}A_{\rm CS} (-i)^{\ell_1+\ell_2+\ell_3}\sum_G (-1)^{\Phi_G} \sum_{\lambda}\sqrt{2\lambda+1} \int 4\pi x^2dx\,\int 4\pi s^2ds\,\sum_{m=1}^2\sum_{l_1l_2l_3l_4}\\\nonumber
    &&\,\times\,\mathcal{Q}^{(1)m}_{\ell_{H1}l_1\lambda}(r_{H1},s,x)\mathcal{Q}^{(2)m}_{\ell_{H2}l_2\lambda}(r_{H2},s,x)\mathcal{Q}^{(3)}_{\ell_{H3}l_3}(r_{H3},s)\mathcal{Q}^{(4)}_{\ell_{H4}l_4}(r_{H4},s)\sum_{L_{12}\ell_1'\ell_2'\ell_3'\ell_4'\ell_{12}'\ell_1''\ell_2''\ell_3''}\\\nonumber
    &&\,\times\,\sum_{\L_0}\mathcal{E}(\L_0)\mathcal{G}^{[l_1l_2(l_{12})l_3l_4][\ell_1'\ell_2'(\ell_{12}')\ell_3'\ell_4']\L_0}\mathcal{G}^{\L_0[\ell_1''\ell_2''(\ell_3'')\ell_3''0][\ell_{H1}\ell_{H2}(L_{12})\ell_{H3}\ell_{H4}]}Z_{\ell_1'}Z_{\ell_2'}Z_{\ell_3'}Z_{\ell_4'}g_{m,\lambda}^{\ell_1''\ell_2''\ell_3''}.
\eeq    
Computation is thus reduced to performing $k$-integrals for each $\ell_i, l_i$, $m$ and $\lambda$, which are then combined via coupled one-dimensional $s$ and $x$ integrals and an angular piece. We further note that the $j_{\ell}(kr)$ terms in \eqref{eq: Q-integrals} can be replaced by bin-averaged spherical Bessel functions \citep[e.g.,][]{2020MNRAS.492.1214P} to incorporate radial binning.

\oliver{can we do the $s$ integral as a sum? probably. May also work for the $x$ integral via Zack's trick?}

